On Tackling the Limits of Resolution in SAT Solving

The practical success of Boolean Satisfiability (SAT) solvers stems from the CDCL (Conflict-Driven Clause Learning) approach to SAT solving. However, from a propositional proof complexity perspective, CDCL is no more powerful than the resolution proof system, for which many hard examples exist. This paper proposes a new problem transformation, which enables reducing the decision problem for formulas in conjunctive normal form (CNF) to the problem of solving maximum satisfiability over Horn formulas. Given the new transformation, the paper proves a polynomial bound on the number of MaxSAT resolution steps for pigeonhole formulas. This result is in clear contrast with earlier results on the length of proofs of MaxSAT resolution for pigeonhole formulas. The paper also establishes the same polynomial bound in the case of modern core-guided MaxSAT solvers. Experimental results, obtained on CNF formulas known to be hard for CDCL SAT solvers, show that these can be efficiently solved with modern MaxSAT solvers.

==> scratch.tex <==
%------------------------------------------------------------------------------%
% File:        scratch.tex
%
% Description: 
%
% Created:     21 Apr 2017.
%
% Author:      Joao Marques-Silva (jpms).
%------------------------------------------------------------------------------%

\section{Short \mxsat Proofs for PHP\hfill[OLD]} \label{sec:proofs}

\subsection{A Polynomial Bound on Core-Guided Algorithms \hfill[OLD]}

To understand how \mxsat can be used for inferring that the
propositional encoding of \php is unsatisfiable, we start by
considering a somewhat idealized execution of a core-guided \mxsat
algorithm. (A working knowledge of the operation of a core-guided
algorithm will help understanding the arguments in this section.)
%
To facilitate the analysis, it is assumed that \atmost1 constraints
are encoded with the pairwise encoding~\cite{sat-handbook09}.
%
%
\begin{table}[t]
  \begin{center}
    \caption{Simplified core-guided unit propagation steps} \label{tab:cg-proof}
    \renewcommand{\arraystretch}{1.25}
    \renewcommand{\tabcolsep}{0.35em}
    \scalebox{0.835}{
      \begin{tabular}{|C{1.5cm}|C{2.75cm}|C{3.125cm}|C{3cm}|C{3cm}|} \hline
        Constraint & Hard clause(s) & Soft clause(s) & Relaxed clauses & Equivalent clause(s)\\
        \hline\hline
      $\fml{L}_i$ &
        $(\neg n_{i1}\lor\ldots\lor\neg n_{im})$ &
        $(n_{i1}), \ldots, (n_{im})$ &
        $(n_{i1}), \ldots, (n_{im})$ &
        $(n_{i1}\lor n_{i2}\lor\ldots\lor n_{im})$
        \\ \hline
        $\fml{M}_j$ &
        $(\neg p_{1j}\lor\neg p_{2j})$ &
        $(p_{1j}),(p_{2j})$ &
        $(p_{1j}),(p_{2j})$ &
        $(p_{1j}\lor p_{2j})$
        \\ \hline
        $\fml{M}_j$ &
        $(\neg p_{1j}\lor\neg p_{3j}),$\newline $(\neg p_{2j}\lor\neg p_{3j})$ &
        $(p_{1j}\lor p_{2j}),(p_{3j})$ &
        $(p_{1j}\lor p_{2j}),(p_{3j})$ &
        $(p_{1j}\lor p_{2j}\lor p_{3j})$
        \\ \hline
        \multicolumn{5}{|c|}{$\cdots$}
        \\ \hline
        $\fml{M}_j$ &
        $(\neg p_{1j}\lor\neg p_{m+1\,j}),$\newline
        $(\neg p_{2j}\lor\neg p_{m+1\,j}),$\newline
        $\ldots$,\newline 
        $(\neg p_{mj}\lor\neg p_{m+1\,j})$ &
        $(p_{1j}\lor\ldots\lor p_{mj}),$\newline$(p_{m+1\,j})$ &
        $(p_{1j}\lor\ldots\lor p_{mj}),$\newline$(p_{m+1\,j})$ &
        $(p_{1j}\lor\ldots\lor p_{m+1\,j})$
        \\ \hline
      \end{tabular}
    }
  \end{center}
\end{table}
%
%
\autoref{tab:cg-proof} summarizes the execution of a core-guided
\mxsat algorithm. The description of the execution of the core-guided
algorithm is simplified by assuming that some clauses are added at
each step, when in fact existing soft clauses are relaxed and
\atmost$k$ constraints are added or updated. (From the perspective of 
the operation of a core-guided \mxsat solver, no difference would be
observed.)
%
For each \atleast1 constraint $\fml{L}_i$, unit propagation yields a
conflict, which results in increasing the lower bound on the number of
falsified soft clauses by 1. Since there are $m+1$ constraints
$\fml{L}_i$, each of which using disjoint sets of variables, the lower
bound can be raised to $m+1$ by relaxing the soft clauses used for
deriving each conflict.

For each \atmost1 constraint $\fml{M}_j$, a total of $m$ conflicts
will be identified. The soft clauses involved in each conflict are
relaxed and an AtMost$k$ constraint is added or updated. Each step can
be viewed as adding a new soft clause, as shown
in~\autoref{tab:cg-proof}. As can be observed in the simpler cases,
each conflict will be identified by unit propagation, using the hard
and soft clauses shown (in reality relaxed clauses would be
considered, but unit propagation would still produce each conflict).
%
As a result, we can conclude that each $\fml{M}_j$ raises by $m$ the
lower bound on the number of falsified soft clauses. Since there are
$m$ constraints $\fml{M}_j$, then the lower bound is raised in $m\cdot
m$, which is to be added to the $m+1$ resulting from the $\fml{L}_i$
constraints. 
%
In total, successive application of unit propagation and relaxation
steps enables raising the lower bound to $m(m+1)+1$. However, this
lower bound is already \emph{above} the target value of $m(m+1)$.
Thus, we have shown that \emph{any} assignment satisfying the hard
clauses of the \hmxsat encoding of \php will falsify at least
$m(m+1)+1$ soft clauses. Thus, we can conclude that the original \php
propositional encoding is unsatisfiable.
%
%
The intuition outlined above will be formalized in the next section,
by showing the \mxsat resolution steps used for deriving $m(m+1)+1$
empty clauses.

\begin{nproposition}
  For a core-guided \mxsat solver, there is a sequence of unit
  propagation steps such that a lower bound of $m(m+1)+1$ is computed
  in polynomial time.
\end{nproposition}

\begin{proof}(Sketch)
  The discussion above.
\end{proof}

It is important to observe that the unit propagation steps consider
avoid the clauses in $\fml{P}$, i.e.\ only the clauses in $\fml{L}_i$,
$\fml{M}_j$, $\fml{S}$, and relaxed clauses, are used for deriving the
lower bound of $m(m+1)+1$ on minimum the number of falsified soft
clauses. As shown in~\autoref{sec:res}, and for the concrete case of
\php, the clauses in $\fml{P}$ are actually unnecessary and actually
impact negatively the performance of core-guided \mxsat solvers.


%------------------------------------------------------------------------------%

